A fast and consistent sharp-interface immersed boundary method for moving bodies of arbitrary thickness

Immersed boundary methods (IBMs) are widely used to simulate flows around complex geometries and moving bodies, but they often involve a trade-off between precision and computational efficiency. Eulerian formulations require special treatments for moving walls and may generate spurious force oscillations, whereas Lagrangian formulations can suffer from slip errors at the immersed surfaces. We propose a novel sharp-interface IBM for incompressible flows involving moving, deformable, and arbitrary-thickness bodies. The method combines a fast tagging algorithm, a two-sided Eulerian forcing strategy, and a consistent mass correction that reduces the splitting error of fractional-step schemes, while preserving the structure of the discrete Laplacian operator. This formulation retains the efficiency of direct Poisson solvers, thus avoiding the overhead of cut-cell, multigrid, and projection-based approaches. The method naturally handles moving boundaries, and yields small transpiration errors with second-order accuracy in the enforcement of the no-slip condition. Numerical tests using rigid, deformable, turbulent, and biologically inspired flows demonstrate the accuracy, robustness, and efficiency of the method, without compromising computational cost.

==> _figures/general/grid_and_surface_double.tex <==
    \def\step{1.2}   
    \def\shift{0.2*\step}   

    \coordinate (OW) at (-1.5*\step  -0.2*\step, 3.15*\step + \shift);
    \coordinate (BW) at (-0.3*\step, 0.4*\step + \shift);
    \coordinate (CW) at ( 2*\step + 0.2*\step, -0.1*\step + \shift);

    \coordinate (Wp)  at ( 0.9*\step,0.1*\step + \shift);
    \coordinate (Wm)  at (-0.8*\step,1.1*\step + \shift);
    
    \coordinate (Fp)  at (0*\step,\step);
    \coordinate (Fm)  at (0*\step,0*\step);

    \coordinate (Wt)  at (-0.15*\step, 0.35*\step + \shift);
    \coordinate (Wb)  at ( 0.15*\step, 0.25*\step + \shift);

    %\node at (-1.4*\step,2.9*\step) [] {$\mathcal{S}$};

    % eulerian grid
    \draw[step=\step, shift={({\step}, {0.0*\step})}] (-3*\step - 0.2*\step, -2.*\step - 0.2*\step) grid (1*\step + 0.2*\step, 3*\step + 0.2*\step);
    \foreach \i in {-2, -1, 0, 1, 2} {
        \foreach \j in {-2,-1, 0, 1, 2, 3} {
            \filldraw[black]  (\i*\step, \j*\step) circle (2pt);
        }
    }
    
    % surface
    \draw [gray , line width = 3pt] plot [smooth] coordinates {(OW) (Wm) (BW) (Wp) (CW)};
    

